DIAL-SUMMER: A Structured Evaluation Framework of Hierarchical Errors in Dialogue Summaries

Dialogues are a predominant mode of communication for humans, and it is immensely helpful to have automatically generated summaries of them (e.g., to revise key points discussed in a meeting, to review conversations between customer agents and product users). Prior works on dialogue summary evaluation largely ignore the complexities specific to this task: (i) shift in structure, from multiple speakers discussing information in a scattered fashion across several turns, to a summary's sentences, and (ii) shift in narration viewpoint, from speakers' first/second-person narration, standardized third-person narration in the summary. In this work, we introduce our framework DIALSUMMER to address the above. We propose DIAL-SUMMER's taxonomy of errors to comprehensively evaluate dialogue summaries at two hierarchical levels: DIALOGUE-LEVEL that focuses on the broader speakers/turns, and WITHIN-TURN-LEVEL that focuses on the information talked about inside a turn. We then present DIAL-SUMMER's dataset composed of dialogue summaries manually annotated with our taxonomy's fine-grained errors. We conduct empirical analyses of these annotated errors, and observe interesting trends (e.g., turns occurring in middle of the dialogue are the most frequently missed in the summary, extrinsic hallucinations largely occur at the end of the summary). We also conduct experiments on LLM-Judges' capability at detecting these errors, through which we demonstrate the challenging nature of our dataset, the robustness of our taxonomy, and the need for future work in this field to enhance LLMs' performance in the same. Code and inference dataset coming soon.

==> tables/prior-taxonomies.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{|p{0.2\textwidth}|p{0.7\textwidth}|p{0.2\textwidth}|}
\toprule
\textbf{Prior taxonomies} & \textbf{Definition} & Mapped to \taxonomy  \\ \midrule
Misreferencing & A property or an event in the summary sentence can be found in the source material, but are associated with the wrong entity &  \\ \midrule
Coreference error & A pronoun or reference with wrong or non-existing antecedent &  \\ \midrule
Linking / Discourse Error & Error in how multiple statements are linked together in the discourse (for example temporal ordering or causal link) & \\ \midrule
Stating opinion as fact & The summary sentence entails a proposition that's mentioned in the source material not as a fact, but as someone’s opinion &  \\ \midrule
Tense/Modality  & The tense or modal (e.g. can, may, must, e.g. might vs. will) used in the summary does not match the tense/modality of the source &  \\ \midrule
Nuanced Meaning Shift & The summary sentence twists information from the source material in a subtle way &  \\ \midrule
Number & A claim has a different number (year, dimensions, ages, dates etc.) than the original context (e.g. 20\% vs. 0.7\%). &  \\ \midrule
Entity & A claim includes swapped, incorrectly specified, or inserted noun phrases &  \\ \midrule
False Concatenation & A claim incorrectly combines information about multiple entities or events &  \\ \midrule
Attribution Failure & A claim lacks proper attribution, either crediting the wrong source or presenting information as fact without citation &  \\ \midrule
Overgeneralization & A claim is based on accurate contextual information but is too broad or too general to be supported by the context. &  \\ \midrule
Reasoning Error & A claim is based on accurate contextual information but contains a reasoning error or makes an unsupported conclusion. &  \\ \midrule
Hyperbole & A claim is based on accurate information but exaggerated or overstated &  \\ \midrule
Context-based meaning & Incorrect interpretation of idiomatic language, homonyms, or words with multiple meanings, failing to capture the intended meaning &  \\ \midrule
Partially supported & The claim is mostly consistent with the source text, but some words are added, omitted, or inaccurate &  \\ \midrule
Unevaluable & The claim cannot be interpreted as a statement to evaluate against the source text (e.g. it is a question or instruction). &  \\ \midrule
Non-factual & Implies whether it aligns with factual information &  \\ \midrule
Incoherence & Includes input-conflicting, context-conflicting and self-conflicting contents in the dialogue &  \\ \midrule
Out-of-Article Error & Summary introduces facts, subjective opinions, or biases that cannot be verified or confirmed by the source text &  \\ \midrule
Relation Error & Incorrect semantic relationships within a summary sentence, such as wrong verbs, prepositions, or adjectives, which misrepresent the relationship between entities &  \\ \midrule
Sentence Error & A summary sentence entirely contradicts the information in the source text, requiring significant revision or removal &  \\ \midrule
Predicate error & The predicate in the summary statement is inconsistent with the document &  \\ \midrule
Circumstantial error & The additional information (like location or time) specifying the circumstance around a predicate is wrong &  \\ \midrule

Grammatical Error & Significant grammatical mistakes & N/A  \\ \bottomrule
\end{tabular}
}
\caption{Errors from prior taxonomies versus ours.}
\label{tab:prior-taxonomy-errors}
\end{table*}
